Single-Photon 3D Imaging with Equi-Depth Photon Histograms

Single-photon cameras present a promising avenue for high-resolution 3D imaging. They have ultra-high sensitivity -- down to individual photons -- and can record photon arrival times with extremely high (sub-nanosecond) resolution. Single-photon 3D cameras estimate the round-trip time of a laser pulse by forming equi-width (EW) histograms of detected photon timestamps. Acquiring and transferring such EW histograms requires high bandwidth and in-pixel memory, making SPCs less attractive in resource-constrained settings such as mobile devices and AR/VR headsets. In this work we propose a 3D sensing technique based on equi-depth (ED) histograms. ED histograms compress timestamp data more efficiently than EW histograms, reducing the bandwidth requirement. Moreover, to reduce the in-pixel memory requirement, we propose a lightweight algorithm to estimate ED histograms in an online fashion without explicitly storing the photon timestamps. This algorithm is amenable to future in-pixel implementations. We propose algorithms that process ED histograms to perform 3D computer-vision tasks of estimating scene distance maps and performing visual odometry under challenging conditions such as high ambient light. Our work paves the way towards lower bandwidth and reduced in-pixel memory requirements for SPCs, making them attractive for resource-constrained 3D vision applications. Project page: $\href{https://www.computational.camera/pedh}{https://www.computational.camera/pedh}$

==> sec/table1.tex <==
\usepackage{multirow}

% Table for middlebury and nyu datasets
\begin{table}[]
\begin{tabular}{rrcccccc}
 &  & \begin{tabular}[c]{@{}c@{}}Conventional SPC \\ (1000 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Conventional SPC\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CSPH {[}?{]}\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PEDH Naive\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PEDH Interpolated\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}DeePEDH {[}Ours{]}\\ (32 bins)\end{tabular} \\ \hline
\multicolumn{2}{r}{\begin{tabular}[c]{@{}r@{}}Bandwidth \\ Required\end{tabular}} & 100Gbps & 0.3Gbps & 0.3Gbps & 0.3Gbps & 0.3Gbps & 0.3Gbps \\
\multirow{4}{*}{\begin{tabular}[c]{@{}r@{}}NYUv2 {[}?{]}\\ Dataset\end{tabular}} & RMSE & 6.890 cm & 29.800 cm & 15.010 cm & 18.050 cm & 18.220 cm & 10.920 cm \\
 & MAE & 1.060 cm & 24.580 cm & 2.030 cm & 2.400 cm & 2.770 cm & 1.840 cm \\
 & 2\% Inliers & 99.893 \% & 10.687 \% & 99.450 \% & 97.870 \% & 95.085 \% & 98.510 \% \\
 & 10\% Inliers & 99.896 \% & 55.855 \% & 99.623 \% & 99.705 \% & 99.705 \% & 99.805 \% \\
\multirow{4}{*}{\begin{tabular}[c]{@{}r@{}}Middlebury {[}?{]}\\ Dataset\end{tabular}} & RMSE & 1.730 cm & 26.920 cm & 2.050 cm & 2.190 cm & 2.710 cm & 2.120 cm \\
 & MAE & 0.780 cm & 23.520 cm & 0.800 cm & 0.920 cm & 1.410 cm & 0.980 cm \\
 & 2\% Inliers & 99.968 \% & 5.2230 \% & 99.958 \% & 99.757 \% & 93.923 \% & 99.220 \% \\
 & 10\% Inliers & 99.970 \% & 36.421 \% & 99.968 \% & 99.968 \% & 99.968 \% & 99.937 \%
\end{tabular}
\end{table}


% Table for NYU dataset only
\begin{table}[]
\begin{tabular}{r|cccccc}
 & \begin{tabular}[c]{@{}c@{}}Conventional SPC \\ (1000 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Conventional SPC\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CSPH {[}?{]}\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PEDH Naive\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PEDH Interpolated\\ (32 bins)\end{tabular} & \begin{tabular}[c]{@{}c@{}}DeePEDH {[}Ours{]}\\ (32 bins)\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}Bandwidth \\ Required\end{tabular} & 100Gbps & 0.3Gbps & 0.3Gbps & 0.3Gbps & 0.3Gbps & 0.3Gbps \\
RMSE & 6.890 cm & 29.800 cm & 15.010 cm & 18.050 cm & 18.220 cm & 10.920 cm \\
MAE & 1.060 cm & 24.580 cm & 2.030 cm & 2.400 cm & 2.770 cm & 1.840 cm \\
2\% Inliers & 99.893 \% & 10.687 \% & 99.450 \% & 97.870 \% & 95.085 \% & 98.510 \% \\
10\% Inliers & 99.896 \% & 55.855 \% & 99.623 \% & 99.705 \% & 99.705 \% & 99.805 \%
\end{tabular}
\end{table}

==> sec/tableA.tex <==
\begin{table}[h]
\vspace{-0.1 in}
{\begin{tabular}{cllll}
\hline
Background flux ($\Phi_\text{bkg}$)                                                      & 0.5 & 1.0 & 2.0 & 5.0  \\ \hline
\begin{tabular}[c]{@{}c@{}}Fixed step (Ref. 16)\end{tabular}      & 6.50 & 7.32 & 9.39 & 10.13  \\
\begin{tabular}[c]{@{}c@{}}Optimized step (Ours)\end{tabular}  & 5.46 & 4.20 & 4.95 & 4.06   \\ \hline
\end{tabular}}
\vspace{-0.07in}
\caption*{{\small{\bf Table T1:} Quantitative metrics for simulated median tracking binners show large improvements in RMSE, faster convergence, and robustness to illumination conditions for optimized stepping.}}
\vspace{-0.15in}
\label{table:3}
\end{table}

==> sec/temp.tex <==


\section{Experimental Details}

Our DeePEDH distance estimator takes the 1024-dimensional density estimates $\rho_1$ as input and predicts the scene distances using the DeepBoosting model \cite{photoneff}. Instead of fine-tuning the model, we train it from scratch on our custom dataset because the distribution of $\rho_1$ is different from what the DeepBoosting model \cite{photoneff} was originally trained on.

\subsection{PEDH Dataset Generation}

We use the dToF imaging model proposed in Eq. (\ref{eq:phihat}) to simulate the photon-timestamp dataset from existing RGB-D datasets \cite{nyuv2, midury}. Previous methods have used a similar model to generate photon timestamp measurements \cite{Lindell1, nonfusiontimeres, photoneff, spadnet, csph}. However, most of them deal with the aggregated EWH output, so they do not need to simulate the photon timestamps for individual laser cycles. In our case, simulating photon timestamps for 1000s of laser cycles is mandatory. Hence, we implement a vectorized, GPU-accelerated photon-timestamp simulator using the PyTorch framework, significantly reducing the experimentation time. 

% We share a detailed runtime comparison of a naive sub-optimal simulator and the vectorized GPU-accelerated simulator for different numbers of pixels.

To simulate the dToF measurements, we assume a Gaussian laser pulse of 100 ns timeperiod and full width at half maximum (FWHM) of 0.32 ns and represent it with a resolution of 1024 time bins similar to other recent work \cite{photoneff, Lindell1}. To simulate the PEDH output, we update the binners for $L = 5000$ laser cycles with the following optimized stepping parameters: $K = 3$, $f_s = 0.8$, $\theta_{clip} = 0.02$, $m_1 = 0.95$ and $m_2 = 0.8$. These parameter values were obtained by performing an exhaustive grid search over a wide range of each hyper parameter and then choosing the combination of values that give the least RMSE in PEDH estimates with respect to OrEDH values. 

\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{Images/Figure 9.png}
\caption{\textbf{Evaluation results on NYU test images} Image showing qualitative results for distance estimation for naive method and DL method highlighting how the naive method can drastically fail for poor SBR scenarios but the DL model is able to learn the spatiotemporal correlations between the PEDH output to improve the distance estimates in extreme conditions.}
\label{fig:distestim_results1}
\end{figure*}

\subsection{Training and validation details}
We train the DeepBoosting model \cite{photoneff} for our DeePEDH distance estimator. We simulate PEDH output for a vast range of scenes and illumination conditions from the NYU-V2 dataset \cite{nyuv2}. The training and validation dataset is generated using the RGB-D images from the NYU-V2 dataset. The training dataset consists of 2K RGB-D images from the official training split of the dataset and the validation dataset consists of 200 RGB-D images from the official test split of the dataset. To make the model robust to different SBR scenarios, we simulate the PEDH output by randomly choosing a pair of average signal and background photons per cycle from the following pairs (1.0, 1.0), (1.0, 2.0), (1.0, 5.0), (0.5, 0.5), (0.5, 1.0), (0.5, 2.5). 

\subsection{Performance evaluation}
We evaluate the performance of the narrowest-bin distance estimator and the DeePEDH distance estimator and compare the results with three baseline methods --- Distance from 1024-bin EWH, distance from 32-bin EWH, and distance from the compressive single-photon histogram (CSPH) method \cite{csph}. We evaluate the performance on two different test sets. The first test set consists of 8 different images from the Middlebury dataset \cite{midury} and the second test set consists of 10 different images from the test set of the NYU-V2 dataset. For each test image, we test the distance estimators for the following eight signal, background photon pairs: (1.0, 1.0), (1.0, 2.0), (1.0, 5.0), (1.0, 10.0),  (0.5, 0.5), (0.5, 1.0), (0.5, 2.5) and (0.5, 5.0). 

% \imp{Should we reduce the number of average signal and background photon values? We increased the number to reduce the simulation time OR the other option is to simply talk in terms of SBR and avoid mentioning the actual signal and background photons?}.

The performance is compared based on four different evaluation metrics:  RMSE, MAE, $1 \%$ inlier metric, and $10 \%$ inlier metric. Fig.~\ref{fig:distestim_results1} shows qualitative and quantitative results for three NYU test images for two different SBRs. The DeePEDH distance estimator shows superior performance over all other methods, especially for poor SBR scenarios. Observe the results for the narrowest-bin method, where the distance estimates for some of the pixels are accurate. The results clearly highlight that the DeePEDH distance estimator is able to exploit spatio-temporal correlations and is able to generalize well on challenging scenarios.

For most of the metrics, the DL method outperforms the rest of the methods. The margin is higher for NYU test images as they contain more challenging scenes. The performance for all methods except the 32 EWH bin is almost similar for the Middlebury test images. 

% \begin{figure*}[h]
% \centering
% \includegraphics[width=\linewidth]{Images/Figure 9.png}
% \caption{\textbf{Evaluation results on NYU test images} Image showing qualitative results for distance estimation for naive method and DL method highlighting how the naive method can drastically fail for poor SBR scenarios but the DL model can learn the spatiotemporal correlations between the PEDH output to improve the distance estimates in extreme conditions.}
% \label{fig:distestim_results1}
% \end{figure*}


\section{PEDH for resource-constrained computer-vision applications}
So far we have shown that the proposed PEDH can generate ED histograms with less bandwidth and in-pixel memory requirements. Hence we may be able to fabricate SPCs using PEDH that are ideal for power and resource-constrained applications, such as autonomous robots, virtual reality headsets, portable 3D scanners, etc. Such computer-vision applications use the scene-distance information as part of their processing pipeline. 

In this section, we explore the question: What if conventional (1024 bin EWH) SPCs were replaced by PEDH-based SPCs in resource-constrained applications?
We show results for two computer vision tasks: RGB-D \textit{visual odometry} (VO) and \textit{Truncated Signed Distance Function} (TSDF) fusion. These tasks are common components of several resource-constrained applications, including ones mentioned above. 

For both applications, we simulate distance estimates from a 32-bin EWH and a 32-bin PEDH so that both use the same amount of memory to store dToF data. The distance estimates are then passed to the respective computation pipelines. We show qualitative results for both the histogrammers.

\subsection{Application 1: RGBD-Visual Odometry}

Visual odometry \cite{odom1, odom2} is the task of estimating camera pose and motion from image sequences captured by the camera. In the case of RGB-D cameras, the sequences consist of RGB images and corresponding distance maps. The key component of a VO pipeline is the feature-matching step where the movement of interesting visual features is estimated between consecutive frames and used to compute the camera trajectory. The quality of distance estimates in each frame directly affects the feature-matching step. For resource-constrained applications there are strict bandwidth and memory limitations that affect the quality of distance measurements and thus the performance of the VO pipeline. 

We simulate distance maps from 32-bin EWH and 32-bin EDH\footnote{To keep the hardware requirements minimal, we use the narrowest-bin distance estimator for the PEDH output but one can use the DeePEDH distance estimator for even better results with dedicated hardware accelerators.} and pass the RGB-D frames to the existing RGB-D VO pipeline using the Open3D library \cite{open3d} in Python. Fig.~\ref{fig:voresults} shows camera trajectories obtained from the VO pipeline using distance maps from both methods. We observe superior performance for the task of visual odometry using distance maps generated from PEDH.

\begin{figure}[htp]
\centering
\includegraphics[width=0.7\linewidth]{Images/Figure11.png}
\caption{\textbf{PEDH SPCs allow better camera tracking}: Figure showing \textcolor{blue}{ground truth (G.T.)} camera trajectory, trajectory estimated from RGB-D visual odometry using \textcolor{green}{32-bin EWH SPC} and using \textcolor{orange}{32-bin PEDH SPC}. Camera-trajectory estimates are better for PEDH SPC and are quite close to the ground truth.}
\label{fig:voresults}
\end{figure}

% \kscomm{A lot of applications including autonomous drones and smartphones use multiple sensors to estimate the camera pose instead of depending on just the visual information. A common alternative is to combine an inertial measurement unit with the camera and use visual-inertial odometry (VIO) for the camera pose estimates. Using VIO one can propose to avoid using distance maps and rather perform VIO using RGB images and inertial measurements.}

\subsection{Application 2: Dense 3D reconstruction}
Dense 3D reconstruction is a popular computer vision task for applications such as virtual reality, digital twining of 3D assets, photo-realistic telepresence, and autonomous mobile robots. Different types of 3D-sensing methods have been explored to capture accurate dense 3D information and SPC-based dToF sensors are a common choice for such applications.

3D reconstruction pipelines have two major components: (i) estimating the camera pose per frame and, (ii) fusing the RGB-D information to reconstruct a 3D scene that is consistent with a maximum number of RGB-D frames and the corresponding camera pose. A common method to fuse the RGB-D information is the TSDF fusion method \cite{tsdf}. We use the same resource constraints as the VO application and use the distance maps from the EWH and PEDH output as input to the distance-estimation pipeline.

Fig.~\ref{fig:tsdf-fusion} shows qualitative results for TSDF fusion using distance maps from EWH and PEDH output. We see that using PEDH output generates significantly better 3D reconstruction of the scene and contains finer details, whereas using EWH measurements results in highly quantized reconstructions. 
\begin{figure}[htpb]
\centering
\includegraphics[width=0.7\linewidth]{Images/Figure10_3DRecon.png}
\caption{\textbf{PEDH SPCs result in better 3D reconstruction}: Figure showing 3D reconstruction obtained from TSDF fusion using distance estimates from 32-bin EWH SPC (left) and 32-bin PEDH SPC (right). Using a 32-bin PEDH results in cleaner, high-fidelity reconstruction.}
\label{fig:tsdf-fusion}
\end{figure}
\subsection{Application 3: RGB-D deep semantic segmentation}
Another popular computer vision task used to understand the semantics of the scene is called semantic segmentation. In semantic segmentation, each pixel of the image is assigned a class label. Multiple deep-learning methods have been proposed in the past that perform semantic segmentation, some only use RGB image \cite{unet,fcn,deeplab,pspnet,segformer} whereas some use the scene distance image in addition to the RGB image \cite{cen,rgbdjmalik,rgbdrcnn,rgbdmutex}. We use the Channel-Exchanging Network (CEN) proposed by Yikai Wang et.al.\cite{cen} to compare the effect of using distance maps from the 32-bin EWH SPC and the 32-bin PEDH SPC, on the task of deep RGB-D semantic segmentation. We use the NYU-v2 dataset as our test set. We generate CEN output using the ground-truth distance map, and distance maps obtained from the 32-bin EWH SPC, and DeePEDH. The CEN output using a ground-truth distance map is used as the ground-truth for the segmentation result to compare the output for the other two cases. Fig.~\ref{fig:rgbdseg} shows the output for all three cases for different scenes and SBR conditions. Overall we observe that segmentation results are more accurate for DeePEDH as compared to the conventional 32-bin EWH SPC.
\begin{figure}[htpb]
\centering
\includegraphics[width=\linewidth]{Images/Figure13.png}
\caption{\textbf{PEDH SPCs result in better 3D reconstruction}: Figure showing 3D reconstruction obtained from TSDF fusion using distance estimates from 32-bin EWH SPC (left) and 32-bin PEDH SPC (right). Using a 32-bin PEDH results in cleaner, high-fidelity reconstruction.}
\label{fig:rgbdseg}
\end{figure}

\section{Conclusion}

In this work, we proposed a resource-efficient method for compressing raw timestamp data captured by single-photon cameras and studied the effect of using compressed measurements for 3D perception in power-and data-constrained applications. We proposed different distance estimators to predict scene distances from the PEDH output. The experimental results highlight that using our proposed PEDH-based SPCs can achieve superior performance over conventional EWH-based SPCs for popular computer vision tasks like distance estimation, visual odometry, and dense 3D reconstruction. The results for the DeePEDH distance estimator highlight the power of using deep-learning to exploit spatiotemporal correlations captured in PEDH output to improve 3D perception in extreme imaging conditions. 

